RadGeoLoc: Radar Geolocalization via Particle Filtering

In real-time autonomous field applications, GNSS is often unreliable and inaccurate. A possible solution is localizing against a prebuilt map like a satellite image, as it is georeferenced and already surveyed. In this work, we localize a spinning radar measurement against overhead RGB imagery with a learned observation model. We use a radar representation pretrained by masked reconstruction and align it to features from a satellite image. A particle filter propagated by radar odometry proposes candidate poses, and our observation model provides a likelihood over these poses. We evaluate our method over 31 distinct routes, over 8 datasets spanning both urban and offroad conditions using only ground radar and a coarse local prior. We also examine the robustness over changing weather using repeated traversals over the same route over 13 months, in both urban and offroad conditions.

==> Makefile <==
# Paper build. No latexmk, no editor extension -- just make.
#
#   make          regenerate tables from PF results, then build root.pdf
#   make quick    build only, skip table regeneration and bibtex
#   make tables   regenerate paper/tables/*.tex from outputs/pf/*/pf_stats.json
#   make warn     show only the warnings worth acting on
#   make watch    rebuild whenever a .tex changes (polls; no inotify here)
#   make clean    remove build intermediates (keeps the pdf)
#   make distclean  also remove the pdf

DOC      := root
REPO     := $(shell cd .. && pwd)
PYTHON   := $(REPO)/../miniconda3/envs/bev-patch-pf/bin/python
TEXFLAGS := -interaction=nonstopmode -file-line-error
TABLES   := $(wildcard tables/*.tex)
SOURCES  := $(DOC).tex $(TABLES)

.PHONY: all quick tables warn watch clean distclean

all: tables $(DOC).pdf

# Numbers come from the PF results, never from hand-editing a .tex.
tables:
	@cd $(REPO) && $(PYTHON) tools/make_tables.py all -o paper/tables/ 2>&1 | sed 's/^/  /'

# Two passes for cross-references; bibtex in between only if a .bib is cited.
$(DOC).pdf: $(SOURCES)
	@echo "==> pass 1"
	@pdflatex $(TEXFLAGS) $(DOC).tex > .build.log 2>&1 || true
	@if grep -q '\\citation' $(DOC).aux 2>/dev/null && ls *.bib >/dev/null 2>&1; then \
	    echo "==> bibtex"; bibtex $(DOC) >> .build.log 2>&1 || true; fi
	@echo "==> pass 2"
	@pdflatex $(TEXFLAGS) $(DOC).tex >> .build.log 2>&1 || true
	@echo "==> pass 3"
	@pdflatex $(TEXFLAGS) $(DOC).tex >> .build.log 2>&1 || true
	@if [ ! -f $(DOC).pdf ]; then \
	    echo; echo "BUILD FAILED:"; grep -E '^[^ ]+:[0-9]+:' .build.log | head -10; exit 1; fi
	@$(MAKE) --no-print-directory warn
	@echo "==> $(DOC).pdf  ($$(du -h $(DOC).pdf | cut -f1), $$(grep -o '\[[0-9]\+' .build.log | tail -1 | tr -d '[') pages)"

quick:
	@rm -f $(DOC).pdf
	@pdflatex $(TEXFLAGS) $(DOC).tex > .build.log 2>&1 || true
	@if [ ! -f $(DOC).pdf ]; then echo "FAILED:"; grep -E '^[^ ]+:[0-9]+:|^! ' .build.log | head; exit 1; fi
	@$(MAKE) --no-print-directory warn

# Only the warnings that matter: things that change the printed page.
warn:
	@ov=$$(grep -c 'Overfull \\hbox' .build.log 2>/dev/null; true); \
	 uc=$$(grep -c "Citation.*undefined" .build.log 2>/dev/null; true); \
	 ur=$$(grep -c "Reference.*undefined" .build.log 2>/dev/null; true); \
	 echo "    overfull hboxes : $$ov"; \
	 echo "    undefined cites : $$uc"; \
	 echo "    undefined refs  : $$ur"; \
	 if [ "$$ov" != "0" ]; then grep 'Overfull \\hbox' .build.log | sed 's/^/      /' | head -5; fi; \
	 if [ "$$uc" != "0" ]; then grep -o "Citation \`[^']*'" .build.log | sort -u | sed 's/^/      /' | head -8; fi

watch:
	@echo "watching $(SOURCES) -- ctrl-c to stop"
	@last=""; while true; do \
	    cur=$$(ls -l --time-style=+%s $(SOURCES) 2>/dev/null | awk '{print $$6}' | sort | tr '\n' ' '); \
	    if [ "$$cur" != "$$last" ]; then last="$$cur"; \
	      echo "--- $$(date +%H:%M:%S) rebuilding"; $(MAKE) --no-print-directory quick; fi; \
	    sleep 2; done

clean:
	@rm -f $(DOC).aux $(DOC).log $(DOC).out $(DOC).bbl $(DOC).blg $(DOC).toc .build.log
	@echo "cleaned intermediates"

distclean: clean
	@rm -f $(DOC).pdf

